Misalignment, Learning, and Ranking: Harnessing Users Limited Attention

In digital health and EdTech, recommendation systems face a significant challenge: users often choose impulsively, in ways that conflict with the platform's long-term payoffs. This misalignment makes it difficult to effectively learn to rank items, as it may hinder exploration of items with greater long-term payoffs. Our paper tackles this issue by utilizing users' limited attention spans. We propose a model where a platform presents items with unknown payoffs to the platform in a ranked list to $T$ users over time. Each user selects an item by first considering a prefix window of these ranked items and then picking the highest preferred item in that window (and the platform observes its payoff for this item). We study the design of online bandit algorithms that obtain vanishing regret against hindsight optimal benchmarks. We first consider adversarial window sizes and stochastic iid payoffs. We design an active-elimination-based algorithm that achieves an optimal instance-dependent regret bound of $O(\log(T))$, by showing matching regret upper and lower bounds. The key idea is using the combinatorial structure of the problem to either obtain a large payoff from each item or to explore by getting a sample from that item. This method systematically narrows down the item choices to enhance learning efficiency and payoff. Second, we consider adversarial payoffs and stochastic iid window sizes. We start from the full-information problem of finding the permutation that maximizes the expected payoff. By a novel combinatorial argument, we characterize the polytope of admissible item selection probabilities by a permutation and show it has a polynomial-size representation. Using this representation, we show how standard algorithms for adversarial online linear optimization in the space of admissible probabilities can be used to obtain a polynomial-time algorithm with $O(\sqrt{T})$ regret.

==> tex/relatedwork.tex <==

\subsection{Further Related Work}
\label{sec:related}
Besides the rich lines of work on stochastic bandits, adversarial bandits and incentivizing exploration, which we discussed in-depth earlier in the introduction, our work is connected to several other streams of research:

\smallskip
\noindent\emph{Learning to rank.} Online learning to rank is a core problem in information retrieval, machine learning, and online platforms.
Many provably efficient algorithms have been proposed for this problem in specific click models, under different feedback structures, and with different objectives. The canonical examples of click models are the well-studied Cascade Model~\citep{kveton2015cascading,zong2016cascading}, Dependent Click Model (with single or multiple clicks)~\citep{katariya2016dcm}, Position-Based Model with
known position bias~\cite{lagree2016multiple}, Window-based Consider-then-Choose users~\cite{ferreira2022learning}, and general click model~\cite{zoghi2017online,lattimore2018toprank}. There are also several works on adversarial models for learning to rank. These settings are the most
similar to the stochastic position-based and document-based
models, but with the additional robustness bought by the
adversarial framework. For example, \cite{radlinski2008learning}
and the follow up work in \cite{slivkins2013ranked} where the
learner’s objective is to maximize the probability that a user
clicks on any item rather than rewarding multiple clicks.
See the survey by \cite{hofmann2011probabilistic} for more details.
\arpit{Add more discussion about technical novelty.}

\smallskip
\noindent\emph{Product ranking in online platforms.} There is also a rich literature on product ranking optimization in the revenue management literature~\citep{derakhshan2022product,abeliuk2016assortment,gallego2020approximation,aouad2021display,asadpour2022sequential,sumida2021revenue,golrezaei2021learning}, which focus on maximizing revenue (i.e., product-weighted objectives), or a combination of revenue and social welfare, or similar other economically justified objectives --- in different contexts with different applications and agendas.

\smallskip
\noindent\emph{Online combinatorial learning}.
Moving beyond online learning to only rank, our work contributes to the rich literature on adversarial oracle efficient online with exact  algorithms~\cite{kalai2005efficient,dudik2020oracle} or approximation algorithms~\cite{kakade2007playing,niazadeh2022online} as the oracle. Our technical approach, especially in the adversarial setting, is also related to online combinatorial optimization~\cite {audibert2014regret}.

\smallskip
\noindent\emph{Online contextual learning}. In this paper, for simplicity, we consider item-dependent payoffs; however, in recommendation system applications where personalization is allowed, the platform can also benefit from user-dependent payoffs through \emph{contextual learning}~\citep{li2010contextual,li2018online,besbes2021contextual,cohen2020feature,leme2018contextual,liu2018contextual,gollapudi2021contextual}. Fitting our paper into this framework, one can think of our approach as a form of contextual learning where user preferences are essentially the context and used by the platform to rank the products; notably, this context changes the way an item is selected in our model, but not the platform rewards upon selection (and hence no cross-learning is happening nor required).\footnote{Considering a fully contextual-model with context-dependent payoffs, and then trying to benefit from cross-learning across the products, is an interesting avenue for future research.}

